Extragradient Preference Optimization (EGPO): Beyond Last-Iterate Convergence for Nash Learning from Human Feedback

Reinforcement learning from human feedback (RLHF) has become essential for improving language model capabilities, but traditional approaches rely on the assumption that human preferences follow a transitive Bradley-Terry model. This assumption fails to capture the non-transitive nature of populational human preferences. Nash learning from human feedback (NLHF), targeting non-transitive preferences, is a problem of computing the Nash equilibrium (NE) of the two-player constant-sum game defined by the human preference. We introduce Extragradient preference optimization (EGPO), a novel algorithm for NLHF achieving last-iterate linear convergence to the NE of KL-regularized games and polynomial convergence to the NE of original games, while being robust to noise. Unlike previous approaches that rely on nested optimization, we derive an equivalent implementation using gradients of an online variant of the identity preference optimization (IPO) loss, enabling more faithful implementation for neural networks. Our empirical evaluations demonstrate EGPO's superior performance over baseline methods when training for the same number of epochs, as measured by pairwise win-rates using the ground truth preference. These results validate both the theoretical strengths and practical advantages of EGPO for language model alignment with non-transitive human preferences.

==> COLM2025/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> draft.tex <==
\section{Preliminaries}



Let $r$ be an arbitrary vector and define
\begin{align*}
    V_\beta (\theta) = \pi_\theta^\top r - \beta \KL (\pi_\theta || \pi_\tref).
\end{align*}
We know $\theta_\beta^\star = \arg\max_\theta V_\beta (\theta) = \theta_\tref + r / \beta$, and then
\begin{align*}
    V_\beta (\theta_\beta^\star) &= \sum_y \frac{1}{Z(\theta)} r(y) \pi_\tref(y) \ee^{r(y) / \beta} - \beta \sum_y \frac{1}{Z(\theta)} \pi_\tref (y) \ee^{r(y) / \beta} \log \frac{\pi_\tref (y) \ee^{r(y)/\beta}}{Z (\theta) \cdot \pi_\tref (y)} \\
    %
    &= \beta \log Z(\theta) \\
    %
    &= \beta \log \left( \sum_y \pi_\tref (y) \ee^{r(y) / \beta} \right).
\end{align*} 


\paragraph{Uniqueness of solution.}
If there are two solutions $\theta_1, \theta_2$, then we can compute
\begin{align*}
    \KL(\pi_{\theta_1} || \pi_{\theta_2}) + \KL(\pi_{\theta_1} || \pi_{\theta_2})
    %
    &= \langle \log \pi_{\theta_1} - \log \pi_{\theta_2}, \pi_{\theta_1} - \pi_{\theta_2} \rangle \\
    %
    &= \langle \theta_1 - \log Z(\theta_1) \II - \theta_2 + \log Z(\theta_2) \II, \pi_{\theta_1} - \pi_{\theta_2} \rangle \\
    %
    &\myeqi \langle \theta_1 - \theta_2, \pi_{\theta_1} - \pi_{\theta_2} \rangle \\
    %
    &= \frac{1}{\beta} (\pi_{\theta_1} - \pi_{\theta_2})^\top \cP (\pi_{\theta_1} - \pi_{\theta_2}) \\
    %
    &\myeqii 0,
\end{align*}
where (i) is by $\langle C \II, p - q \rangle = 0$ where $p, q \in \Delta^{\cY}$;
(ii) is by $\cP + \cP^\top = \II$ and $\II (p - q) = \vec{0}$ where $p, q \in \Delta^{\cY}$.
This means $\pi_{\theta_1} = \pi_{\theta_2}$ and hence $\theta_1 = \theta_2$.







\paragraph{Transfer KL-divergence.}
In high-level, I want to use a halving sequence of $\beta$s, and adapt the final policy of $\beta$ to an initial policy of $\beta / 2$.
This requires to derive a bound of $\KL (\pi_{\beta/2}^\star || \pi' )$ given $\KL (\pi_\beta^\star || \pi)$.
We write
\begin{align*}
    \theta_\tref = \lambda \left( \theta_\beta^\star - \frac{\cP \pi_\beta^\star}{\beta} \right) + (1 - \lambda) \left( \theta_{\beta/2}^\star - 2 \frac{\cP \pi_{\beta/2}^\star}{\beta} \right).
\end{align*}
Take update
\begin{align*}
    \theta' = (1 - \eta \beta) \theta + \eta \beta \left( \theta_\tref + c \frac{\cP z}{\beta} \right).
\end{align*}
Expanding terms, we have a term
\begin{align*}
    \eta \cP [\lambda \pi_\beta^\star + 2 (1 - \lambda) \pi_{\beta/2}^\star - c z].
\end{align*}
If $0 = \lambda + 2 (1 - \lambda) - c = 2 - \lambda - c$, then we have
\begin{align*}
    [\lambda \pi_\beta^\star + 2 (1 - \lambda) \pi_{\beta/2}^\star - c z]^\top \cP^\top [\lambda \pi_\beta^\star + 2 (1 - \lambda) \pi_{\beta/2}^\star - c z] = 0,
\end{align*}
hence
\begin{align*}
    \langle \theta' - (1 - \eta \beta) \theta - \eta \beta [\lambda \theta_\beta^\star + (1 - \lambda) \theta_{\beta/2}^\star ] , \lambda \pi_\beta^\star + 2 (1 - \lambda) \pi_{\beta/2}^\star - c z \rangle = 0
\end{align*}

\begin{align*}
    \KL (\pi_{\gamma \beta}^\star || \pi_\beta^\star) + \KL (\pi_\beta^\star || \pi_{\gamma \beta}^\star)
    %
    &= \langle \theta_{\gamma \beta}^\star - \theta_\beta^\star, \pi_{\gamma \beta}^\star - \pi_\beta^\star \rangle \\
    %
    &= \left\langle \frac{1}{\gamma \beta} \cP \pi_{\gamma \beta}^\star - \frac{1}{\beta} \cP \pi_\beta^\star, \pi_{\gamma \beta}^\star - \pi_\beta^\star \right\rangle \\
    %
    &= \frac{1}{\beta} \left(\frac{1}{\gamma} - 1\right) (\pi_{\gamma \beta}^\star - \pi_\beta^\star)^\top \cP \pi_{\gamma \beta}^\star + \frac{1}{\beta} (\pi_{\gamma \beta}^\star - \pi_\beta^\star)^\top \cP (\pi_{\gamma \beta}^\star - \pi_\beta^\star) \\
    %
    &= \frac{1}{\beta} \left(\frac{1}{\gamma} - 1\right) (\pi_{\gamma \beta}^\star - \pi_\beta^\star)^\top \cP \pi_{\gamma \beta}^\star.
\end{align*}


\subsection{Newton's Method}

\todorz{quasi-Newton, BFGS, backtracking line search}

Let $F(\theta) := \theta - \theta_\tref - \frac{\cP \pi_\theta}{\beta}$.
Take the update
\begin{align*}
    \theta^{(t+1)} = \theta^{(t)} - [J_F (\theta^{(t)})]^{-1} F(\theta^{(t)})
\end{align*}
where $J_F$ is the Jacobian matrix:
\begin{align*}
    J_F (\theta) = I - \frac{\cP (\diag (\pi_\theta) - \pi_\theta \pi_\theta^\top)}{\beta}.
\end{align*}
\todorz{Is this full rank for any $\beta$ and $\theta$? At least for $\theta_\beta^\star$?}

Define the $2$nd order derivative of $F$ by:
\begin{align*}
    (H_F (\theta))_{i, j, k} = \frac{\partial^2 F_i (\theta)}{\partial \theta_j \partial \theta_k}.
\end{align*}
From Taylor's expansion,
\begin{align*}
    F (\theta + \delta) = F(\theta) + J_F (\theta) \delta + \delta^\top \odot H_F (\theta) \odot \delta + \vec{o} (\norm{\delta}_2^2).
\end{align*}
From $F (\theta_\beta^\star) = \vec{0}$ we have
\begin{align*}
    \theta^{(t+1)} - \theta_\beta^\star &= \theta^{(t)} - \theta_\beta^\star - [J_F (\theta^{(t)})]^{-1} [F(\theta^{(t)}) - F(\theta_\beta^\star)] \\
    %
    &= \theta^{(t)} - \theta_\beta^\star - [J_F (\theta^{(t)})]^{-1} [J_F (\theta^{(t)}) (\theta^{(t)} - \theta_\beta^\star) - (\theta^{(t)} - \theta_\beta^\star)^\top \odot H_F (\theta^{(t)}) \odot (\theta^{(t)} - \theta_\beta^\star) + \vec{o} (\norm{\theta^{(t)} - \theta_\beta^\star}_2^2)] \\
    %
    &= [J_F (\theta^{(t)})]^{-1} (\theta^{(t)} - \theta_\beta^\star)^\top \odot H_F (\theta^{(t)}) \odot (\theta^{(t)} - \theta_\beta^\star) + [J_F (\theta^{(t)})]^{-1} \vec{o} (\norm{\theta^{(t)} - \theta_\beta^\star}_2^2).
\end{align*}


\paragraph{Approximating the inverse.}
We use a basic identity here: for an invertible matrix $A$ and a constant $c$ such that $-I \prec I - cA \prec I$, we have that
\begin{align*}
    A^{-1}=c (c A)^{-1} = c \sum_{n=0}^\infty (I - c A)^n.
\end{align*}
Let $A = J_F (\theta)$, then we need to find $c$ such that
\begin{align*}
    I - c \left(I - \frac{\cP (\diag (\pi_\theta) - \pi_\theta \pi_\theta^\top)}{\beta} \right)
\end{align*}
converges for the summation.
\todorzout{How to characterize this for a non-symmetric matrix?}


We begin by the identity of matrix inverse:
\begin{align*}
    (I - U V)^{-1} = I + U (I - V U)^{-1} V.
\end{align*}
Let $U = \cP / \beta$ and $V = \diag (\pi_\theta) - \pi_\theta \pi_\theta^\top$, we have
\begin{align*}
    [J_F (\theta)]^{-1} = I + \frac{1}{\beta} \cP \left(I + \frac{(\diag (\pi_\theta) - \pi_\theta \pi_\theta^\top) \cP}{\beta} \right)^{-1} (\diag (\pi_\theta) - \pi_\theta \pi_\theta^\top).
\end{align*}
From $\cP + \cP^\top = \II$, we have
\begin{align*}
    I + \frac{(\diag (\pi_\theta) - \pi_\theta \pi_\theta^\top) \cP}{\beta}
    %
    &= I + \frac{(\diag (\pi_\theta) - \pi_\theta \pi_\theta^\top) (\II - \cP^\top)}{\beta} \\
    %
    &\myeqi I - \frac{(\diag (\pi_\theta) - \pi_\theta \pi_\theta^\top) \cP^\top}{\beta} \\
    %
    &= [J_F (\theta)]^\top,
\end{align*}
where (i) is by \red{$(\diag (\pi_\theta) - \pi_\theta \pi_\theta^\top) \II = \vec{0}$}.


Let $\cL (\theta) = \norm{F(\theta)}_2^2$.
Then $\nabla \cL (\theta) = 2 [J_F (\theta)]^\top F (\theta)$.



We have
\begin{align*}
    \theta^{(t+1)} &= \theta^{(t)} - 2 \eta [J_F (\theta^{(t)})]^\top \Sigma (\samp) F(\theta^{(t)}), \\
    %
    \theta^{(t+1)} - \theta_\beta^\star &= \theta^{(t)} - \theta_\beta^\star - 2 \eta [J_F (\theta^{(t)})]^\top \Sigma (\samp) [F(\theta^{(t)}) - F(\theta_\beta^\star)] \\
    %
    &= \left(I - 2 \eta [J_F (\theta^{(t)})]^\top \Sigma (\samp) J_F (\theta^{(t)}) \right) (\theta^{(t)} - \theta_\beta^\star) \\
    %
    &\quad + 2 \eta [J_F (\theta^{(t)})]^\top \Sigma (\samp) (\theta^{(t)} - \theta_\beta^\star)^\top \odot H_F (\theta^{(t)}) \odot (\theta^{(t)} - \theta_\beta^\star)\\
    %
    &\quad + \vec{o} (\norm{\theta^{(t)} - \theta_\beta^\star}_2^2)
\end{align*}

Let $\zeta$ be any parameter vector and $z$ be any distribution.
We first propose an update in the form of
\begin{align}
    \theta^{(t+1)} = \theta^{(t)} - 2 \eta [J_F (\zeta)]^\top \Sigma (\samp) \left(\theta^{(t)} - \theta_\tref - \frac{\cP z}{\beta} \right). \label{eq:any_update_precond}
\end{align}
This is a preconditioned version of \Cref{eq:any_update}.
We would like to derive a similar equation as \Cref{eq:update_inner_product}:
\begin{align}
    & \langle \theta^{(t+1)} - (I - 2 \eta [J_F (\zeta)]^\top \Sigma (\samp)) \theta^{(t)} - 2 \eta [J_F (\zeta)]^\top \Sigma (\samp) \theta_\beta^\star, [[J_F (\zeta)]^\top \Sigma (\samp)]^{-1} (\pi_\beta^\star - z) \rangle \notag \\
    %
    &= - \frac{2 \eta}{\beta} \langle [J_F (\zeta)]^\top \Sigma (\samp) \cP (\pi_\beta^\star - z), [[J_F (\zeta)]^\top \Sigma (\samp)]^{-1} (\pi_\beta^\star - z) \rangle \notag \\
    %
    &= - \frac{2 \eta}{\beta} (\pi_\beta^\star - z)^\top \cP (\pi_\beta^\star - z) \notag \\
    %
    &= 0. \label{eq:update_inner_product_precond}
\end{align}


\begin{align*}
    \nabla (u^\top \pi_\theta) = [J_\pi (\theta)]^\top u
\end{align*}



For log-linear policy, $f_\theta (y) = (\Phi \theta)_y$, then $J_f (\theta) = \Phi$.
So $\nabla_\theta \cL_\ipo (\theta; \sg{\pi_\theta}) = 2 \Phi^\top \Sigma (\samp) F(\theta) \approx \frac{2}{\abs{\cY}} \Phi^\top F(\theta)$ where
$F(\theta) = \Phi \theta - \Phi \theta_\tref - \frac{\cP \pi_\theta}{\beta}$.
However, for extragradient, we desire
\begin{align*}
    \theta^{(t+1/2)} \gets \theta^{(t)} - \eta \beta (\Phi^\top \Phi)^\dagger \Phi^\top F(\theta^{(t)}) \approx \theta^{(t)} - \frac{\eta \beta \abs{\cY}}{2} \{[J_f (\theta^{(t)})]^\top J_f (\theta^{(t)})\}^\dagger \nabla_\theta \cL_\ipo (\theta; \sg{\pi_\theta}).
\end{align*}
If we assume $\Phi_{i, j} \sim \cN (0, 1 / \sqrt{\abs{\cY}})$, then $\bbE [\Phi^\top \Phi] = I$.
$\theta^{(t+1/2)}$ is the minimizer of
\begin{align*}
    [\nabla_\theta \cL_\oipo (\theta^{(t)})]^\top (\theta - \theta^{(t)}) + \frac{1}{\eta \beta \abs{\cY}} (\theta - \theta^{(t)})^\top [J_f (\theta^{(t)})]^\top J_f (\theta^{(t)}) (\theta - \theta^{(t)}).
\end{align*}
This could be transformed into constrained optimization:
\begin{align*}
    \textup{maximize} [\nabla_\theta \cL_\oipo (\theta^{(t)})]^\top (\theta - \theta^{(t)}), \textup{subject to }
\end{align*}
\todorz{Can similar idea of PPO be used here?}


==> trash.tex <==
From \Cref{eq:update_inner_product,eq:extragrad_est1},
\begin{align*}
    \KL (\pi^{(t)} || \pi^{(t+1/2)}) - \eta \beta \KL (\pi^{(t)} || \pi_\beta^\star) - \KL (\pi_\beta^\star || \pi^{(t+1)}) + (1 - \eta \beta) \KL (\pi_\beta^\star || \pi^{(t)}) = 0.
\end{align*}

The following relation holds:
\begin{align*}
    \KL (\pi^{(t)} || \pi^{(t+1)})
    %
    &= \langle \log \pi^{(t)} - \log \pi^{(t+1/2)}, \pi^{(t)} \rangle + \langle \log \pi^{(t+1/2)} - \log \pi^{(t+1)}, \pi^{(t+1/2)} \rangle \\
    %
    &\quad + \langle \log \pi^{(t+1/2)} - \log \pi^{(t+1)}, \pi^{(t)} - \pi^{(t+1/2)} \rangle \\
    %
    &\myeqi \KL (\pi^{(t)} || \pi^{(t+1/2)}) + \KL (\pi^{(t+1/2)} || \pi^{(t+1)}) + \eta (\pi^{(t)} - \pi^{(t+1/2)})^\top \cP (\pi^{(t)} - \pi^{(t+1/2)}) \\
    %
    &\myeqii \KL (\pi^{(t)} || \pi^{(t+1/2)}) + \KL (\pi^{(t+1/2)} || \pi^{(t+1)}),
\end{align*}
where (i) is by \Cref{eq:extragrad_est1,eq:extragrad_upd};
(ii) is by $\cP + \cP^\top = \II$ and $(p - q)^\top \II (p - q) = 0$.


By definition,
\begin{align*}
    \KL (\pi^{(t+1)} || \pi_\beta^\star)
    %
    &\le \KL (\pi^{(t+1)} || \pi_\beta^\star) + \KL (\pi_\beta^\star || \pi^{(t+1)}) \\
    %
    &= \langle \log \pi^{(t+1)} - \log \pi_\beta^\star, \pi^{(t+1)} - \pi_\beta^\star \rangle \\
    %
    &= \underbrace{\langle \theta^{(t+1)} - \theta_\beta^\star, \pi^{(t+1)} - \pi_\beta^\star \rangle}_{=: f_{t+1}}.
\end{align*}
We compute the recursive relation on $f$.
\begin{align*}
    f_{t+1} &\myeqi (1 - \eta \beta) \langle \theta^{(t)} - \theta_\beta^\star, \pi^{(t+1)} - \pi_\beta^\star \rangle + \eta (\pi^{(t+1)} - \pi_\beta^\star)^\top \cP  (\pi^{(t+1/2)} - \pi_\beta^\star) \\
    %
    &= (1 - \eta \beta) (f_t + \underbrace{\langle \theta^{(t)} - \theta_\beta^\star, \pi^{(t+1)} - \pi^{(t)} \rangle}_{=: g_{t+1}}) + \eta (\pi^{(t+1)} - \pi_\beta^\star)^\top \cP  (\pi^{(t+1/2)} - \pi_\beta^\star) \\
    %
    &\myleii (1 - \eta \beta) (f_t + g_{t+1}) + \eta (\KL (\pi_\beta^\star || \pi^{(t+1)}) / \sqrt{\eta \beta} + \sqrt{\eta \beta} \KL (\pi^{(t+1/2)} || \pi_\beta^\star)) \\
    %
    &\myleiii (1 - \eta \beta) (f_t + g_{t+1}) + 2 \eta \sqrt{\frac{\eta}{\beta}} (1 - \eta \beta)^t \KL (\pi_\beta^\star || \pi^{(0)}),
\end{align*}
where (i) is by \Cref{eq:extragrad_upd} and $\theta_\beta^\star = (1 - \eta \beta) \theta_\beta^\star + \eta \beta (\theta_\tref + \cP \pi_\beta^\star / \beta)$;
(ii) is by \Cref{lem:diff_quad_form} with $\xi = 1 / \sqrt{\eta \beta}$;
(iii) is by \Cref{eq:extragrad_kl,eq:extragrad_est_rev_kl}.
Meanwhile,
\begin{align*}
    g_{t+1} &= \langle \theta^{(t)} - \theta^{(t+1)}, \pi^{(t+1)} - \pi^{(t)} \rangle + \langle \theta^{(t + 1)} - \theta_\beta^\star, \pi^{(t+1)} - \pi^{(t)} \rangle \\
    %
    &=-\KL(\pi^{(t)} || \pi^{(t+1)}) - \KL(\pi^{(t+1)} || \pi^{(t)}) + \langle \theta^{(t + 1)} - \theta_\beta^\star, \pi^{(t+1)} - \pi^{(t)} \rangle \\
    %
    &\mylei (1 - \eta \beta) g_{t+1} + \eta (\pi^{(t+1)} - \pi^{(t)})^\top \cP (\pi^{(t+1/2)} - \pi_\beta^\star) \\
    %
    &= (1 - \eta \beta) g_{t+1} + \eta (\pi^{(t+1)} - \pi_\beta^\star)^\top \cP (\pi^{(t+1/2)} - \pi_\beta^\star) + \eta (\pi_\beta^\star - \pi^{(t)})^\top \cP (\pi^{(t+1/2)} - \pi_\beta^\star) \\
    %
    &\myleii (1 - \eta \beta) g_{t+1} + \eta (\KL (\pi_\beta^\star || \pi^{(t+1)}) / \sqrt{\eta \beta} + \sqrt{\eta \beta} \KL (\pi^{(t+1/2)} || \pi_\beta^\star)) + \eta (\KL (\pi_\beta^\star || \pi^{(t)}) / \sqrt{\eta \beta} + \sqrt{\eta \beta} \KL (\pi^{(t+1/2)} || \pi_\beta^\star)) \\
    %
    &\myleiii (1 - \eta \beta) g_{t+1} + 4 \eta \sqrt{\frac{\eta}{\beta}} (1 - \eta \beta)^t \KL (\pi_\beta^\star || \pi^{(0)}),
\end{align*}
where (i) is by \Cref{eq:extragrad_upd} and $\theta_\beta^\star = (1 - \eta \beta) \theta_\beta^\star + \eta \beta (\theta_\tref + \cP \pi_\beta^\star / \beta)$;
(ii) is by \Cref{lem:diff_quad_form} with $\xi = 1 / \sqrt{\eta \beta}$;
(iii) is by \Cref{eq:extragrad_kl,eq:extragrad_est_rev_kl}.
So we have
\begin{align*}
    g_{t+1} \le 4 \sqrt{\frac{\eta}{\beta^3}} (1 - \eta \beta)^t \KL (\pi_\beta^\star || \pi^{(0)}).
\end{align*}
The recursion on $f$ is then
\begin{align*}
    f_{t+1} \le (1 - \eta \beta) f_t + 4 \sqrt{\frac{\eta}{\beta^3}} (1 - \eta \beta)^t \KL (\pi_\beta^\star || \pi^{(0)}).
\end{align*}
Solving it yields
\begin{align*}
    f_t \le \left( f_0 + \frac{4}{1 - \eta \beta} \sqrt{\frac{\eta}{\beta^3}} \KL (\pi_\beta^\star || \pi^{(0)}) \cdot t \right) (1 - \eta \beta)^t.
\end{align*}
Plugging into \Cref{lem:dual_gap} yields the desired result:
\begin{align*}
    &\dualgap_\beta (\pi^{(T)}) \\
    %
    &\le \frac{2}{\beta} \KL(\pi_\beta^\star || \pi^{(T)}) + 2 \beta \KL (\pi^{(T)} || \pi_\beta^\star) \\
    %
    &\le \frac{2}{\beta} (1 - \eta \beta)^T \KL(\pi_\beta^\star || \pi^{(0)}) + 2 \beta \left( \KL (\pi_\beta^\star || \pi^{(0)}) + \KL (\pi^{(0)} || \pi_\beta^\star) + \frac{4}{1 - \eta \beta} \sqrt{\frac{\eta}{\beta^3}} \KL (\pi_\beta^\star || \pi^{(0)}) \cdot T \right) (1 - \eta \beta)^T \\
    %
    &\le \left[2 \beta \KL (\pi^{(0)} || \pi_\beta^\star) + \left( \frac{2}{\beta} + 2 \beta + \frac{8}{1 - \eta \beta} \sqrt{\frac{\eta}{\beta}} T \right) \KL (\pi_\beta^\star || \pi^{(0)}) \right] (1 - \eta \beta)^T.
\end{align*}


\subsubsection{OMWU}

We can also change \Cref{eq:extragrad_est1} into
\begin{align}
    \theta^{(t+1/2)} &= (1 - \eta \beta) \theta^{(t)} + \eta \beta \left(\theta_\tref + \frac{\cP \pi^{(t-1/2)}}{\beta} \right). \label{eq:extragrad_est2}
\end{align}
Then
\begin{align*}
    \theta^{(t+1/2)} - \theta^{(t+1)}
    %
    &= \eta \cP (\pi^{(t)} - \pi^{(t+1/2)}) + \eta \cP (\pi^{(t-1/2)} - \pi^{(t)}), \\
    %
    \langle \theta^{(t+1/2)} - \theta^{(t+1)}, \pi^{(t+1/2)} - \pi^{(t+1)} \rangle
    %
    &\le \eta \left( \KL( \pi^{(t)} || \pi^{(t+1/2)}) + \KL(\pi^{(t-1/2)} || \pi^{(t)}) + 2 \KL(\pi^{(t+1)} || \pi^{(t+1/2)}) \right).
\end{align*}
So
\begin{align*}
    \KL (\pi_\beta^\star || \pi^{(t+1)})
    %
    &\le (1 - \eta \beta) \KL (\pi_\beta^\star || \pi^{(t)}) - \eta \beta \KL (\pi^{(t+1/2)} || \pi_\beta^\star) + \eta \KL (\pi^{(t)} || \pi^{(t-1/2)})  \\
    %
    &\quad - (1 - \eta \beta - \eta ) \KL (\pi^{(t+1/2)} || \pi^{(t)}) - (1 - 2 \eta) \KL (\pi^{(t+1)} || \pi^{(t+1/2)}) \\
\end{align*}
If $1 - \eta \beta - \eta \ge 0$ and $(1 - \eta \beta) (1 - 2 \eta) \ge \eta$, i.e., \red{$\eta \le \frac{1}{\beta + 1}$ and $\eta \in (0, (\beta + 3 - \sqrt{\beta^2 - 10 \beta + 9}) / (8 \beta)] \cup [ (\beta + 3 + \sqrt{\beta^2 - 10 \beta + 9}) / (8 \beta), +\infty)$}, we have
\begin{align*}
    \KL (\pi_\beta^\star || \pi^{(t+1)}) + (1 - 2 \eta) \KL (\pi^{(t+1)} || \pi^{(t+1/2)})
    %
    \le (1 - \eta \beta) [\KL (\pi_\beta^\star || \pi^{(t)}) + (1 - 2 \eta) \KL (\pi^{(t)} || \pi^{(t-1/2)})],
\end{align*}
which also implies a linear convergence of $\KL (\pi_\beta^\star || \pi^{(t+1)})$.





The practical implementation of the extragradient update is in the pseudo code (\Cref{alg:practical_extragrad}).
\begin{algorithm}[tb]
    \caption{Practical Implementation of the Extragradient Update}
    \label{alg:practical_extragrad}
    \begin{algorithmic}
        \STATE {\bf Input:} number of update $T$, sampling policy $\samp$, reference policy $\pi_\tref$, preference model $\cP$.
        \STATE Initialize $\pi \gets \pi_\tref$.
        \FOR{$t=1,2,\ldots,T$}
            \STATE $\pi$.zero\_grad() and scheduler.step().
            \STATE Sample two independent pairs $(y_t, y_t') \sim \samp$ and $(y_{t+1/2}, y_{t+1/2}') \sim \samp$.
            \STATE Evaluate using $\pi$ and $\pi_\tref$:
            \begin{align*}
                h_t = \log \frac{\pi (y_t) \pi_\tref (y_t')}{\pi (y_t') \pi_\tref (y_t)}, \quad
                %
                h_{t+1/2} = \log \frac{\pi (y_{t+1/2}) \pi_\tref (y_{t+1/2}')}{\pi (y_{t+1/2}') \pi_\tref (y_{t+1/2})}.
            \end{align*}
            \STATE Sample $y_t'' \sim \pi$.
            \STATE Sample / evaluate $I(y_t, y_t'')$ and $I(y_t', y_t'')$ using $\cP$.
            \STATE Calculate loss: $\cL_t = \left(h_t - \frac{I(y_t, y_t'') - I(y_t', y_t'')}{\beta} \right)^2$.
            \STATE $\cL_t$.backward() and optimizer.step().
            \STATE \red{Store the model parameter: $g \gets$ optimizer.grad.}
            \STATE Sample $y_{t+1/2}'' \sim \pi$.
            \STATE Sample / evaluate $I(y_{t+1/2}, y_{t+1/2}'')$ and $I(y_{t+1/2}', y_{t+1/2}'')$ using $\cP$.
            \STATE Calculate loss: $\cL_{t+1/2} = \red{-}\left(h_{t+1/2} - \frac{I(y_{t+1/2}, y_{t+1/2}'') - I(y_{t+1/2}', y_{t+1/2}'')}{\beta} \right)^2$.
            \STATE \red{optimizer.negate\_LR().}
            \STATE $\cL_{t+1/2}$.backward() and optimizer.step().
            \STATE \red{optimizer.negate\_LR().}
        \ENDFOR
    \end{algorithmic}
\end{algorithm}
